Gigs with Guarantees: Achieving Fair Wage for Food Delivery Workers

With the increasing popularity of food delivery platforms, it has become pertinent to look into the working conditions of the 'gig' workers in these platforms, especially providing them fair wages, reasonable working hours, and transparency on work availability. However, any solution to these problems must not degrade customer experience and be cost-effective to ensure that platforms are willing to adopt them. We propose WORK4FOOD, which provides income guarantees to delivery agents, while minimizing platform costs and ensuring customer satisfaction. WORK4FOOD ensures that the income guarantees are met in such a way that it does not lead to increased working hours or degrade environmental impact. To incorporate these objectives, WORK4FOOD balances supply and demand by controlling the number of agents in the system and providing dynamic payment guarantees to agents based on factors such as agent location, ratings, etc. We evaluate WORK4FOOD on a real-world dataset from a leading food delivery platform and establish its advantages over the state of the art in terms of the multi-dimensional objectives at hand.

==> related.tex <==
\section{Related work}
\noindent {\bf Food order assignment: } 
In the realm of food delivery, most existing work includes unreasonable assumptions, such as having perfect information about orders arrival~\cite{article:mealDelivery}, neglecting the road network~\cite{mdrp}, and skipping the time it takes to prepare food~\cite{10.14778/3368289.3368297}. Joshi et al. ~\cite{foodmatch} addresses all these issues and provides a realistic and scalable solution. \textcolor{blue}{Some recent work provides various frameworks for assigning delivery agents to orders while optimizing delivery times and platform cost per order \cite{Paul2020AnOF,Kottakki2020CustomerED,Ulmer2021TheRM}, distributing delivery agents in different parts of the city to ensure demand and supply are balanced\cite{Xue2021OptimizationOR}, and minimizing delivery agents' waiting time\cite{Weng2021LaborrightPD}}. ~\cite{fairfoody} showed huge payment-based fairness issues due to the one-sided optimization used in the allocation scheme adopted by \cite{foodmatch}. \cite{fairfoody} proposes a multi-objective algorithm to ensure fairly distributed income opportunities among the agents and minimal increase delivery times. Allocation algorithms used in the cab-hailing industry are not adaptable in food delivery, as discussed in \cite{foodmatch}.
\vspace{1mm}
\noindent {\bf Fairness in multi-sided platform algorithms: }
Few studies have looked at how producers and customers interact on two-sided platforms. In matching scenarios, Chakraborty et al. \cite{Chakraborty2017FairSF} and  Suhr et al. \cite{suhr2019two} offered solutions for two-sided fairness. Burke et al.\cite{Burke} classified different types of multi-stakeholder platforms based on their required group fairness characteristics. \cite{Patro_2020} addresses individual fairness for producers and buyers in two-sided platforms with personalized suggestions.  
Despite these efforts to improve fairness in two-sided platforms, only \cite{fairfoody} looks fairness aspect in food delivery platforms without providing any minimum wage guarantee for delivery agents.

